Analysis of Distributed Deep Learning in the Cloud

We aim to resolve this problem by introducing a comprehensive distributed deep learning (DDL) profiler, which can determine the various execution "stalls" that DDL suffers from while running on a public cloud. We have implemented the profiler by extending prior work to additionally estimate two types of communication stalls - interconnect and network stalls. We train popular DNN models using the profiler to characterize various AWS GPU instances and list their advantages and shortcomings for users to make an informed decision. We observe that the more expensive GPU instances may not be the most performant for all DNN models and AWS may sub-optimally allocate hardware interconnect resources. Specifically, the intra-machine interconnect can introduce communication overheads up to 90% of DNN training time and network-connected instances can suffer from up to 5x slowdown compared to training on a single instance. Further, we model the impact of DNN macroscopic features such as the number of layers and the number of gradients on communication stalls. Finally, we propose a measurement-based recommendation model for users to lower their public cloud monetary costs for DDL, given a time budget.

==> 5.implementation.tex <==
\section{Implementation} \label{sections: implementation}

\name builds on top of DS-analyzer to facilitate the profiling of interconnect and network stalls.
% To measure interconnect stalls, \name launches a single synthetic training process in a multi-GPU setup.
% \name is also augmented with capabilities to profile multi-node training to aid in network stall measurement.
% \textcolor{red}{\name also contains synthetic models to "augment" stall behavior in order to learn the QoS properties of a particular machine.}
% \name also comes packaged with a recommendation tool that suggests near-optimal configurations consisting of AWS P instances for a particular user-provided model under a given cost and/or time budget.
We discuss the implementation details of \name below.

\subsection{Profiler details}

\name is written in python and uses the PyTorch \cite{pytorch} framework for deep learning in both standard and distributed data parallel modes to 
respectively support single and multi-node \textcolor{red}{(multi-worker)} training.
\name generates synthetic data according to the user's input and launches 
DDL through multiple training processes.
Since \name adheres to the data parallel deep learning paradigm, each training process works only on a subset of the training data.
However, during step 1, \name deliberately launches a single process on one worker (GPU) so as to measure the training time without inter-GPU communication overhead.
To support profiling of multi-node training scenarios, the user must run their training through \name in all machines and provide distributed PyTorch parameters (such as the master IP address and node "rank").
The user can then run \name on a node with an equivalent number of GPUs to calculate network stalls.
We provide analysis scripts to calculate all stalls (including multi-node) along with visualizations in the \name source code.
The script also calculates the monetary cost of training depending on region-based pricing and the utilization of resources such as GPU, CPU, etc.

\subsection{Synthetic models}

\subsection{Recommendation tool}



==> 9.ack.tex <==
\section*{Acknowledgements}\label{sections: ack}
This research was supported in part by NSF CNS grant 2122155
and ...

==> authors.tex <==
% \begin{comment}

% \author{
% \centering
% \IEEEauthorblockN{ Aakash Sharma}
% \IEEEauthorblockA{\textit{Dept. of Electrical Engineering and Computer Science} \\
% \textit{Pennsylvania State University}\\
% University Park, PA \\
% abs5688@psu.edu}\\
% %\and
% \centering
% \IEEEauthorblockN{Saravanan Dhakshinamurthy}
% \IEEEauthorblockA{
% \textit{Facebook, Inc.}\\
% Menlo Park, CA \\
% saravanand@fb.com}\\
% %\and
% \centering
% \IEEEauthorblockN{Chita R. Das}
% \IEEEauthorblockA{\textit{Dept. of Electrical Engineering and Computer Science} \\
% \textit{Pennsylvania State University}\\
% University Park, PA \\
% cxd12@psu.edu}\\
% %\and
% \centering
% \IEEEauthorblockN{George Kesidis}
% \IEEEauthorblockA{\textit{Dept. of Electrical Engineering and Computer Science} \\
% \textit{Pennsylvania State University}\\
% University Park, PA \\
% gik2@psu.edu}\
% }
% \end{comment}


%  \author{
%     \IEEEauthorblockN{
%      Aakash Sharma\IEEEauthorrefmark{1},
%      Saravanan Dhakshinamurthy\IEEEauthorrefmark{2},
%      George Kesidis\IEEEauthorrefmark{1},
%      Chita R. Das\IEEEauthorrefmark{1},
%      }

%     \IEEEauthorblockA{
%      \IEEEauthorrefmark{1}The Pennsylvania State University, University Park \IEEEauthorrefmark{2} Facebook Inc. \vspace{2mm}
%      }
% }

% \author{\IEEEauthorblockN{Aakash Sharma\IEEEauthorrefmark{1}, George Kesidis\IEEEauthorrefmark{1}, Chita R. Das\IEEEauthorrefmark{1}}
% \IEEEauthorblockA{\IEEEauthorrefmark{1} Computer Science and Engineering, The Pennsylvania State University, \IEEEauthorrefmark{2} Facebook Inc.} %State College, USA\\}
% \{abs5688, gik2, das\}@psu.edu,
% \vspace{-2mm}}
